Decidability of Non-Interactive Simulation of Joint Distributions

We present decidability results for a sub-class of "non-interactive" simulation problems, a well-studied class of problems in information theory. A non-interactive simulation problem is specified by two distributions $P(x,y)$ and $Q(u,v)$: The goal is to determine if two players, Alice and Bob, that observe sequences $X^n$ and $Y^n$ respectively where $\{(X_i, Y_i)\}_{i=1}^n$ are drawn i.i.d. from $P(x,y)$ can generate pairs $U$ and $V$ respectively (without communicating with each other) with a joint distribution that is arbitrarily close in total variation to $Q(u,v)$. Even when $P$ and $Q$ are extremely simple: e.g., $P$ is uniform on the triples $\{(0,0), (0,1), (1,0)\}$ and $Q$ is a "doubly symmetric binary source", i.e., $U$ and $V$ are uniform $\pm 1$ variables with correlation say $0.49$, it is open if $P$ can simulate $Q$. In this work, we show that whenever $P$ is a distribution on a finite domain and $Q$ is a $2 \times 2$ distribution, then the non-interactive simulation problem is decidable: specifically, given $\delta > 0$ the algorithm runs in time bounded by some function of $P$ and $\delta$ and either gives a non-interactive simulation protocol that is $\delta$-close to $Q$ or asserts that no protocol gets $O(\delta)$-close to $Q$. The main challenge to such a result is determining explicit (computable) convergence bounds on the number $n$ of samples that need to be drawn from $P(x,y)$ to get $\delta$-close to $Q$. We invoke contemporary results from the analysis of Boolean functions such as the invariance principle and a regularity lemma to obtain such explicit bounds.

==> sec_agdist.tex <==
\section{Generalized Agreement Distillation}\label{sec:gen_ag_dist}

Cannonne et al. \cite{CGMS_ISR} -- using a result of \cite{bogdanov2011extracting} -- showed that for any $\epsilon > 0$, if Alice and Bob are given access to i.i.d. samples from $\DSBS(\epsilon)$, then, \emph{perfectly agreeing} on $k$ random samples requires $\Omega_{\epsilon}(k)$ bits of communication. In this section, we show that a stronger version of their statement holds. Namely, for any $\epsilon > 0$ and $\epsilon' \gg \epsilon \cdot \log(1/\epsilon)$, if Alice and Bob are given access to i.i.d. samples from $\DSBS(\epsilon')$, then, generating $k$ random samples from $\DSBS(\epsilon)$ requires $\Omega_{\epsilon,\epsilon'}(k)$ bits of communication. Before formally stating the main result of this section, we start by recalling the definition of the Agreement Distillation task that was studied, in particular, by \cite{CGMS_ISR}. Recall that for any random variable $X$, its \emph{min-entropy} $H_{\infty}(X)$ is defined as $H_{\infty}(X) := \min_x(\log(\frac{1}{\Pr[X=x]}))$.

\begin{defn}[Agreement Distillation; \cite{CGMS_ISR}]
In the AgreementDistillation$_{\gamma}^k$ problem, Alice and Bob have no inputs. Their goal is to output $w_A$ and $w_B$ satisfying the following properties:
\begin{enumerate}
\item[(i)] $\Pr[w_A=w_B] \geq \gamma$.
\item[(ii)] $H_{\infty}(w_A) \geq k$.
\item[(iii)] $H_{\infty}(w_B) \geq k$.
\end{enumerate}
\end{defn}

We generalize this definition as follows:
\begin{defn}[Generalized Agreement Distillation]
In the AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$ problem, Alice and Bob have no inputs. Their goal is to output $w_A, w_B \in \{0,1\}^k$ satisfying the following properties:
\begin{enumerate}
\item[(i)] $\Pr[\Delta(w_A,w_B) \le \epsilon k] \geq \gamma$.
\item[(ii)] $H_{\infty}(w_A) \geq \alpha \cdot k$.
\item[(iii)] $H_{\infty}(w_B) \geq \alpha \cdot k$.
\end{enumerate}
\end{defn}

We are now ready to state the main statement of this section.
\begin{lem}\label{le:gen_ag_dist_with_com}
For any $\gamma > 0$, if Alice and Bob are given access to i.i.d. samples from $\DSBS(\epsilon')$, then any interactive protocol solving AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$ should communicate at least
$$ k \cdot (\Omega(\alpha \cdot \epsilon') - H_b(\epsilon)) - \log(1/\gamma) ~~~ \text{ bits.}$$

\end{lem}

In the rest of this section, we prove Lemma~\ref{le:gen_ag_dist_with_com}. We start with the next two lemmas about Generalized Agreement Distilliation. Lemma~\ref{le:ham_ball_chernoff} -- which follows from the Chernoff bound -- says that if Alice and Bob are given access to i.i.d. samples from $\DSBS(\epsilon)$, then they can generate two length-$k$ binary strings that lie in a Hamming ball of radius $\approx \epsilon k$ with high probability. Lemma~\ref{le:gen_ag_dist_imposs} says that agreeing on two such strings is impossible if Alice and Bob are given access of i.i.d. samples from $\DSBS(\epsilon')$ where $\epsilon' \gg \epsilon \cdot \log(1/\epsilon)$.
\begin{lem}\label{le:ham_ball_chernoff}
Let $0 < \delta < \epsilon$. Given access to i.i.d samples from $\DSBS(\epsilon-\delta)$, one can solve the AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$ problem with $\gamma = 1-\exp(-(\epsilon-\delta)^2 \cdot k)$ and $\alpha = 1$.
\end{lem}

\iffalse
\begin{proof}
Follows by applying the Chernoff bound.
\end{proof}
\fi

\begin{lem}\label{le:gen_ag_dist_imposs}
Given access to (infinitely many) i.i.d. samples from $\DSBS(\epsilon')$, there is no zero-communication protocol solving the AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$ problem with
$$ \gamma > 2^{-k \cdot (\frac{\alpha \cdot \epsilon'}{2-\epsilon'}-H_b(\epsilon)) + 1} $$
\end{lem}

\begin{proof}
We will use the following small-set expansion property of the noisy hypercube.

\begin{theorem}[Generalized Small-Set Expansion Theorem; Section $10.1$ of \cite{o2014analysis}]\label{thm:gen_sse}
Let $0 \le \rho \le 1$. Let $A,B \subseteq \{\pm 1\}^n$ have volumes $\exp(-\frac{a^2}{2})$ and $\exp(-\frac{b^2}{2})$ respectively, and assume that $0 \le \rho a \le b \le a$. Then,
$$ \Pr_{x \sim_{\rho} y} [x \in A, y \in B] \le \exp(-\frac{1}{2} \frac{a^2 - 2\rho a b + b^2}{1-\rho^2}) $$
\end{theorem}

We fix $\rho > 0$ and we assume that there is a zero-communication protocol solving  AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$. Without loss of generality, such a protocol is given by two functions $\Ext_A: \{ \pm1 \}^m \to \{ \pm 1 \}^k$ for some integer $m \in \mathbb{N}$. We denote $w_A := \Ext_A(r)$ and $w_B := \Ext_B(r')$ where the coordinates of $r,r' \in \{ \pm 1 \}^m$ are sampled i.i.d from $\DSBS(\epsilon)$. For every $z \in \{ \pm 1 \}^k$, we denote $A_z := \Ext_A^{-1}\{z\}$ and $B_z := \Ext_B^{-1}\{z\}$. Since $H_{\infty}(w_A) \geq \alpha k$ and $H_{\infty}(w_B) \geq \alpha k$, we get that for every $z \in \{ \pm 1 \}^k$, $|A_z|, |B_z| \le 2^{m-\alpha k}$. Thus, the volumes of $A_z$ and $B_z$ are given by:
$$ \frac{|A_z|}{2^m} = \exp(-\frac{a_z^2}{2})$$
$$ \frac{|B_z|}{2^m} = \exp(-\frac{b_z^2}{2})$$
with $a_z, b_z \geq \sqrt{2 \alpha k \ln{2}}$.

We fix $z,z' \in \{ \pm 1 \}^k$ and assume for now that $|A_z| \le |B_{z'}|$; the case where $|A_z| > |B_{z'}|$ is symmetric. If $a_z \geq b_{z'} \geq \rho a_z$, Theorem~\ref{thm:gen_sse} yields that
$$ \Pr_{r \sim_{\rho} r'}[\Ext_A(r) = z, \Ext_B(r') = z'] = \Pr_{r \sim_{\rho} r'}[r \in A_z, r' \in B_{z'}] \le \exp(-\frac{1}{2} \frac{a_z^2 - 2 \rho a_z b_{z'} + b_{z'}^2}{1-\rho^2})$$
and so
$$ \Pr[\Ext_A(r) = z ~ | ~ \Ext_B(r') = z'] \le \exp(-\frac{1}{2} \frac{a_z^2 - 2 \rho a_z b_{z'} + \rho^2 b_{z'}^2}{1-\rho^2}) \le \exp(-\frac{b_{z'}^2}{2} \frac{1-\rho}{1+\rho}) \le 2^{- \alpha k \frac{1-\rho}{1+\rho}},$$
where the penultimate inequality follows from the fact that $a_z \geq b_{z'}$. On the other hand, when $\rho a_z \geq b_{z'} \geq 0$, we can upper bound the probability as
$$ \Pr_{r \sim_{\rho} r'}[r \in A_z, r' \in B_{z'}] \le \Pr_{r}[r \in A_z] \le \exp(-\frac{b_{z'}^2}{2\rho^2}) $$
and
$$ \Pr[\Ext_A(r) = z ~ | ~ \Ext_B(r') = z'] \le \exp(-\frac{1-\rho^2}{2 \rho^2} b_{z'}^2) \le \exp(-\frac{1-\rho}{1+\rho}\cdot \frac{b_{z'}^2}{2}) \le 2^{-\alpha k \frac{1-\rho}{1+\rho}}.$$
A similar (symmetric in $a_z$ and $b_{z'}$) bound holds in the case where $|B_{z'}| \le |A_z|$. Therefore, we have that
\begin{align*}
&\Pr_{r \sim_{\rho} r'}[\Delta(\Ext_A(r), \Ext_B(r')) \le \epsilon k]\\ 
&= \displaystyle\sum\limits_{z \in \{ \pm 1 \}^k} \Pr_{(r,r')}[\Ext_A(r) = z, \Ext_B(r') \in \Ball(z,\epsilon k)]\\ 
&\le \displaystyle\sum\limits_{z \in \{ \pm 1 \}^k \atop z' \in \Ball(z,\epsilon k)}  \Pr_{(r,r')}[\Ext_A(r) = z, \Ext_B(r') = z']\\ 
&\le \displaystyle\sum\limits_{z, z' \in \{ \pm 1 \}^k: \atop \Delta(z,z') \le \epsilon k}  \Pr_{(r,r')}[ r \in A_z, r' \in B_{z'}]\\ 
&\le \displaystyle\sum\limits_{\substack{z,z' \in \{ \pm 1 \}^k: \\ \Delta(z,z') \le \epsilon k \\ a_z \geq b_{z'}}}  \Pr_{(r,r')}[ r \in A_z, r' \in B_{z'}] + \displaystyle\sum\limits_{\substack{z,z' \in \{ \pm 1 \}^k: \\ \Delta(z,z') \le \epsilon k \\ a_z < b_{z'}}}  \Pr_{(r,r')}[ r \in A_z, r' \in B_{z'}]\\ 
&=  \displaystyle\sum\limits_{\substack{z,z' \in \{ \pm 1 \}^k: \\ \Delta(z,z') \le \epsilon k \\ a_z \geq b_{z'}}}  \Pr[ r \in A_z ~ | ~ r' \in B_{z'}] \cdot \Pr[r' \in B_{z'}] + \displaystyle\sum\limits_{\substack{z,z' \in \{ \pm 1 \}^k: \\ \Delta(z,z') \le \epsilon k \\ a_z < b_{z'}}}  \Pr[r' \in B_{z'} ~ | ~ r \in A_z] \cdot \Pr[r \in A_z]\\ 
&\le \displaystyle\sum\limits_{\substack{z' \in \{ \pm 1 \}^k: \\ z \in \Ball(z',\epsilon k) \\ a_z \geq b_{z'}}}  2^{-\alpha k \frac{1-\rho}{1+\rho}} \cdot \Pr[r' \in B_{z'}] + \displaystyle\sum\limits_{\substack{z \in \{ \pm 1 \}^k: \\ z' \in \Ball(z,\epsilon k) \\ a_z < b_{z'}}} 2^{-\alpha k \frac{1-\rho}{1+\rho}} \cdot \Pr[r \in A_z]\\ 
&\le 2^{H_b(\epsilon)k -\alpha k \frac{1-\rho}{1+\rho}+1}\\ 
&=  2^{-(\alpha k \frac{1-\rho}{1+\rho}-H_b(\epsilon)k-1)}
\end{align*}
where the last inequality above follows by a union bound along with the facts that $| \Ball(z,\epsilon k) | \le 2^{H_b(\epsilon) k}$ for any $z \in \{ \pm 1 \}^k$, and $\sum_{z \in \{ \pm 1\}^k} \Pr_{r}[r \in A_z]= \sum_{z' \in \{ \pm 1\}^k} \Pr_{r'}[r' \in A_{z'}] = 1$. The statement of Lemma~\ref{le:gen_ag_dist_imposs} now follows by setting $\rho = 1-\epsilon'$.
\end{proof}

\noindent We are now ready to prove Lemma~\ref{le:gen_ag_dist_with_com}.

\begin{proofof}{Lemma~\ref{le:gen_ag_dist_with_com}}
Assume that $\Pi$ is a $c$-bit interactive protocol solving the AgreementDistillation$_{\gamma,\epsilon,\alpha,k}$ problem and let $w_A$ and $w_B$ be the output strings that are produced under this protocol by Alice and Bob respectively. Note that we can think of Alice's ``input'' under $\Pi$ as being the random string $r_A \in \{0,1\}^t$, and we can think of Bob's ``input'' as being the random string $r_B \in \{0,1\}^t$, where $(r_A,r_B)$ is a sequence of i.i.d. samples from $\DSBS(\epsilon')$ and $t$ is some positive integer. Note that $\Pi$ partitions the input space $\{0,1\}^t \times \{0,1\}^t$ into $2^c$ \emph{rectangles} (i.e., sets of the form $R = P \times Q$ with $P, Q \subseteq \{0,1\}^t$). By an averaging argument, we get that there should exist a rectangle $R$ such that $\Pr[\Delta(w_A,w_B) \le \epsilon k, \Pi \in R] \geq \gamma/2^c$. Henceforth, we fix this rectangle $R$. We now define the following ``zero-communication'' protocol $\Pi'$. When Alice's random string is $r_A$ and Bob's random string is $r_B$,
\begin{itemize}
\item If there is an $r_B'$ such that $(r_A,r_B') \in R$, then, Alice sets her output string $w_A$ to the output determined by $r_A$ and $R$ under $\Pi$.
\item Otherwise, Alice samples her output string $w_A$ uniformly at random from $\{0,1\}^k$.
\end{itemize}
Bob generates his output string $w_B$ in a similar fashion. We now argue that the protocol $\Pi'$ solves the AgreementDistillation$_{\gamma/2^c,\epsilon,\alpha/2,k}$ problem. By our choice of the rectangle $R$, we have that under $\Pi'$, $\Pr[\Delta(w_A,w_B) \le \epsilon k] \geq \gamma/2^c$. We still need to argue that $H_{\infty}(w_A) \geq \alpha k/2$ (the argument showing that $H_{\infty}(w_B) \geq \alpha k/2$ will be symmetric). Let $w \in \{0,1\}^k$. Under $\Pi'$, we have that
\begin{align*}
\Pr[w_A = w] &= \Pr[W_A = w, \Pi \in R] + \Pr[W_A = w, \Pi \notin R]\\ 
&\le 2^{-\alpha k} + \Pr[\Pi \notin R]\cdot\Pr[W_A = w ~ | ~ \Pi \notin R]\\ 
&\le 2^{-\alpha k} + \Pr[W_A = w ~ | ~ \Pi \notin R]\\ 
&= 2^{-\alpha k} + 2^{-k}\\ 
&\le 2^{-\alpha k/2}
\end{align*}
Hence, we get that $H_{\infty}(w_a) \geq \alpha k/2$. Using Lemma~\ref{le:gen_ag_dist_imposs}, we conclude that we should have that
$$\gamma \cdot 2^{-c} > 2^{-k \cdot (\frac{\alpha \cdot \epsilon'}{2(2-\epsilon')}-H_b(\epsilon)) + 1},$$
which means that we should have $c = k \cdot (\Omega(\alpha \cdot \epsilon') - H_b(\epsilon)) - \log(1/\gamma)$.
\end{proofof}

==> sec_minbisec.tex <==
\mycomment{We might want to replace the precise definitions in the next paragraph by a high-level description, and move the precise definitions to a later section..}
It turns out that Non-Interactive Simulation can be reformulated as a problem about \emph{graph powers} which has a similar flavor to several classical problems in graph theory and theoretical computer science. We describe this connection next. Consider a bipartite weighted graph $G = (L,R,E,\mu)$ where each edge $(u,v) \in E$ is associated a non-negative weight $\mu(u,v)$ and the edge weights sum up to $1$. Moreover, the edge weights induce weights on the vertices by setting $\mu_L(u) := \sum_{v \in R: (u,v) \in E} \mu(u,v)$ for every $u \in L$, and similarly $\mu_R(v) := \sum_{u \in L: (u,v) \in E} \mu(u,v)$ for every $v \in R$. We note that $\mu$ can be interpreted as a probability distribution on $E$, with its marginals on $L$ and $R$ being $\mu_L$ and $\mu_R$ respectively. A \emph{bipartite bisection} of $G$ is a cut $S \subseteq L \cup R$ such that $\mu_L(L \cap S)\approx 1/2$ and $\mu_R(R \cap S) \approx 1/2$, and its cost is $\mu(S \times \overline{S})$. The \emph{minimum bipartite bisection} value of $G$, denoted $\val(G)$, is the minimum cost of a bipartite bisection of $G$.\\ 
Given two weighted bipartite graphs $G = (L,R,E,\mu)$ and $H = (L',R',E',\mu')$, we define their tensor product $G \otimes H = (L \times L', R \times R', E'',\mu'')$ where for every $(u,v) \in E$ and $(u',v') \in E'$, we have that $((u,u'),(v,v')) \in E''$, and $\mu''((u,u'),(v,v')) := \mu(u,v) \cdot \mu'(u',v')$. We then define the \emph{tensor powers} $\{G^{\otimes t}: t \in \mathbb{N}\}$ of graph $G$ inductively by setting $G^{\otimes t} := G \otimes G^{\otimes (t-1)}$ for every integer $t \geq 2$, and setting $G^{\otimes 1} := G$. We now observe that
\begin{equation}\label{eq:min_bis_pwr}
\DSBS(G) = \lim_{t \to \infty} \val(G^{\otimes t})
\end{equation}
We point out that \emph{asymptotic graph power} quantities such as the RHS of Equation~(\ref{eq:min_bis_pwr}) have been investigated in a variety of contexts in graph theory and theoretical computer science \cite{alon2002graph}. In many of these cases, the computatibility of the corresponding asymptotic quantity is not known. One notable example is the \emph{Shannon capacity of a graph} \cite{shannon1956zero,lovasz1979shannon} the computability of which is a well-known open question \cite{alon2006shannon}.

\mycomment{In Equation (\ref{eq:min_bis_pwr}) above, we need to define the notation ``$\DSBS(G)$''.}
